Quantum Speedup for Graph Sparsification, Cut Approximation and Laplacian Solving

Graph sparsification underlies a large number of algorithms, ranging from approximation algorithms for cut problems to solvers for linear systems in the graph Laplacian. In its strongest form, "spectral sparsification" reduces the number of edges to near-linear in the number of nodes, while approximately preserving the cut and spectral structure of the graph. In this work we demonstrate a polynomial quantum speedup for spectral sparsification and many of its applications. In particular, we give a quantum algorithm that, given a weighted graph with $n$ nodes and $m$ edges, outputs a classical description of an $\epsilon$-spectral sparsifier in sublinear time $\tilde{O}(\sqrt{mn}/\epsilon)$. This contrasts with the optimal classical complexity $\tilde{O}(m)$. We also prove that our quantum algorithm is optimal up to polylog-factors. The algorithm builds on a string of existing results on sparsification, graph spanners, quantum algorithms for shortest paths, and efficient constructions for $k$-wise independent random strings. Our algorithm implies a quantum speedup for solving Laplacian systems and for approximating a range of cut problems such as min cut and sparsest cut.

==> header.tex <==

% \usepackage{amssymb,amsthm,amsmath}
\usepackage{braket}
\usepackage{xcolor}
% \usepackage{algorithm}
\usepackage{graphicx}
% \usepackage[noend]{algpseudocode}
% \usepackage{algorithmicx}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
 
% Load package at the end in order to avoid the redefinition of the footnote command
% \usepackage[hidelinks, final=true,colorlinks = false,allcolors = {blue}]{hyperref}
 
% \newtheorem{theorem}{Theorem}
% \newtheorem{proposition}{Proposition}
% \newtheorem{lemma}{Lemma}
% \newtheorem{corollary}{Corollary}
% \newtheorem{definition}{Definition}
\newtheorem{fact}{Fact}
% \newtheorem{claim}{Claim}
 
\newcommand{\tG}{\widetilde{G}}
\newcommand{\tE}{\tilde{E}}
\newcommand{\tw}{\tilde{w}}
\newcommand{\tl}{\tilde{l}}
\newcommand{\tR}{\widetilde{R}}
\newcommand{\val}{\mathrm{val}}
\newcommand{\V}{\mathcal{V}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\E}{\mathcal{E}}
\DeclareMathOperator{\Exp}{\mathbb{E}}
\DeclareMathOperator{\poly}{\mathrm{poly}}
\DeclareMathOperator{\polylog}{\mathrm{polylog}}
\let\mod\relax
\DeclareMathOperator{\mod}{\mathrm{mod}}
 
\newcommand{\tO}{\widetilde{O}}
\newcommand{\Id}{\mathbb{I}}
\newcommand{\Hi}{\mathcal{H}}
\newcommand{\complex}{\mathbb{C}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\integer}{\mathbb{Z}}
\renewcommand{\natural}{\mathbb{N}}
 
\newcommand{\mincut}{\textsc{min\;cut}}
\newcommand{\minstcut}{\textsc{min} $st$-\textsc{cut}}
\newcommand{\maxcut}{\textsc{max\;cut}}
\newcommand{\spcut}{\textsc{sparsest\;cut}}
\newcommand{\balsep}{\textsc{balanced\;separator}}
\newcommand{\minfind}{\textsc{minfind}}
\newcommand{\qspars}{{\normalfont\textbf{Quantum\,Sparsify}}}
\newcommand{\halfspars}{{\normalfont\textbf{Half\,Sparsify}}}
\newcommand{\spanner}{{\normalfont\textbf{Spanner}}}
\newcommand{\cost}{\mathrm{cost}}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\spt}{{\normalfont\textbf{SPT}}}
\newcommand{\tcov}{\tau_{\mathrm{cov}}}
\newcommand{\findb}{\mathrm{FindBits}}
\newcommand{\ORf}{\mathrm{OR}}

% fix lack of algorithmicx package
\newcommand{\State}{\STATE}
\newcommand{\For}{\FOR}
\newcommand{\EndFor}{\ENDFOR}
\newcommand{\If}{\IF}
\newcommand{\EndIf}{\ENDIF}
\newcommand{\Else}{\ELSE}
\newcommand{\While}{\WHILE}
\newcommand{\EndWhile}{\ENDWHILE}
 
\hyphenation{Page-Rank}
